Digital Contact Tracing: Large-scale Geolocation Data as an Alternative to Bluetooth-based Apps' Failure

The currently deployed contact-tracing mobile apps have failed as an efficient solution in the context of the COVID-19 pandemic. None of them has managed to attract the number of active users required to achieve an efficient operation. This urges the research community to re-open the debate and explore new avenues that lead to efficient contact-tracing solutions. This paper contributes to this debate with an alternative contact-tracing solution that leverages already available geolocation information owned by BigTech companies with very large penetration rates in most countries adopting contact-tracing mobile apps. Moreover, our solution provides sufficient privacy guarantees to protect the identity of infected users as well as precluding Health Authorities from obtaining the contact graph from individuals.

==> BTvsGPS.tex <==
\section{BlueTooth Vs smartphone location for contact-tracing}

In this section we present pros and cons of the use of BlueTooth and smartphone's geolocation data in the context of COVID-19 contact-tracing. We again remind that we believe the best option is using both of them in parallel. 

The first condition to decide which technology could be a better fit for contact-tracing is to have a clear understanding regarding how the COVID-19 is transmitted. Unfortunately, experts have not yet agreed on how the virus is transmitted \cite{COVIDAir4}. The only certainty is that the virus is transmitted in short-range distances (i.e., 2m) via droplet direct contact. However, some recent studies suggest that the virus can be also transmitted through indirect contact such as airbone transmission and contaminated object \cite{COVIDair1}. Researchers from Aalto university recently delivered a 3D visualization of a virus travelling model after a person cough or sneeze in a supermarket \cite{Covidair2}. The results suggest that the cloud generated could remain active up to 6 minutes after the cough or sneeze.  Even worse, another recent study \cite{Covidair3} concludes: \textit{"Our results indicate that aerosol and fomite transmission of SARS-CoV-2 is plausible, since the virus can remain viable and infectious in aerosols for hours and on surfaces up to days (depending on the inoculum shed")}. 

BT maximum transmission range varies significantly depending on the environment and specific BT version \cite{BlueToothRange}. It outdoor and industrial environments BT can reach more than 150m, whereas in indoor environments such us home or offices it is limited to less than 50m. It is important to note that for some versions and implementations the maximum reach is much lower. Therefore, we can roughly assume that BT approximately allows tracing contact from 0 to 150m. 

In the case of smartphones different technologies are used for outdoor and indoor location. 

Outdoor location is mostly retrieved using GPS that provides an average accuracy of 4.9m in smartphones-enable devices . Recent advances reported by the Federal Aviation Administration (FAA) reported GPS accuracy below 1.9m in 95\% of the cases with GPS devices. Similarly, high-end users boost GPS accuracy with dual-frequency receivers and/or augmentation systems, which can enable real-time positioning within a few centimeters \cite{GPSAccuracy}. In this discussion we will use the 4.9m GPS accuracy as reference. 

For indoor location smartphones mostly rely in Wifi-based location. To this end the first condition is to know the location of WiFI Access Points the smartphone is receiving signal from. Some vendors of indoor Wifi-Location systems report that the accuracy ranges between 5m and 15m \cite{WifiIndoor}, but according to Google \textit{"if you measure the distance to three or more access points, you can use a multilateration algorithm to estimate the device position that best fits those measurements. The result is typically accurate within 1-2 meters."} \cite{WifiIndoorGoogle}. Large companies like Apple or Google know the position of many WiFi access points, especially in homes and in popular indoor environments such as malls, leisure spaces, sport stadiums, etc. Therefore, in this discussion we will assume that in many popular locations smartphones' location accuracy will be lower than 10m. 

Finally, it is important to highlight smartphones incorporate information from embedded sensors (e.g., accelerometer, gyroscope, etc) to further improve the location accuracy both indoor and outdor spaces \cite{AndroidYouTube}. Therefore, we are probably underestimating the actual accuracy of smartphones' location. Even more, location measures in smartphones are provided together with an estimated error. This may allow LPs discarding locations including large errors.

Based on all this information, for direct-contact virus transmission BT is superior since it can guarantee detecting contacts separated less than 2m both in indoor and outdoor locations.  The D3-PT [REF] protocol for BT contact-tracing proposes to include signal power measures along with the contact detected that allows estimating the actual distance between the smartphone receiving the signal and the smartphone emitting the signal. However, BT is useless in case it is required tracing indirect contact. For instance, if an infected person enters in a restaurant we should be able to trace people that has been in the same restaurant some time after the infected person has left. BT contact-tracing is useless for those cases.

In contrast, smartphones' data may be insufficient in many cases to trace direct contacts below 2m both in outdoor and indoor spaces. Still we could think of quite a few scenarios  where smpartphones' data may be a good proxy for tracing direct contact as well since in some spaces the WiFI+Sensor location technology may be accurate enough to go below the 2m threshold. Even more, experts may decide that if GPS/Wifi information reports that two persons have stood together for several minutes within a short distance (e.g, 4-5m), that case should be considered a risky contact as well. Moreover, smartphones' location data is appropriate to trace indirect contact. For instance, in the example exposed above smartphone data could identify what users have accessed the restaurant after the infected user left in whatever period defined by virus propagation experts (e.g., 10 min, 30 min, 1 hour). 

The ideal scenario in the short-term would be that BT contact-tracing apps are massively installed and used by citizens, and, at the same time, LPs massively compute contact-tracing based on smartphones' location data. That would maximize the chances of retrieving enough contacts to take the necessary actions to test citizens with higher probability of being infected.

The reality is that BT contact-tracing is still not ready in most countries and nobody is able to answer what is the strategy for massive installation of apps. Contrary, massive smartphones' location data is readily in LPs. Until BT contact-racing becomes a feasible option, we advocate for an immediate collaboration between public administrations and LPs to exploit smartphones' location information for (direct and indirect) contact tracing. This paper proposes a simple solution to accomplish that collaboration incorporating high privacy provisions to guarantee the contact tracing is achieved without  revealing citizens location information to public administration nor allowing LPs to infer the identity of infected individuals.



==> FB_base.tex <==
\section{Overview of potential user base from a major Location Provider}
\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{./Figures/FB_MAU.png}
  \caption{XXXXX}
  \label{fig:FB_MAU}
\end{figure}

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{./Figures/FB_DAU.png}
  \caption{XXXXX}
  \label{fig:FB_DAU}
\end{figure}

This section aims to understand what is the potential user base from a major potential Location Provider such as Facebook. We focus in Facebook because we can leverage its Marketing API to retrieve the number of Monthly Active Users (MAU) and Daily Active Users (DAU) in the Facebook ecosystem per LP Provider that will serve to validate the importance of exploring the potential of LP to effectively contribute to the contact tracing task.
FB reports per country and the total population per country retrieved from XXXX [REF]. Figure \ref{fig:FB_DAU} presents the penetration based on DAU values instead.  

FB accounts for 227 territories classified as countries. In 132 (58\%) the penetration considering the reported MAU is higher than 50\%, and 174 (76,6\%) is higher than 25\%. If we consider the DAU, 49 (21.6\%) and 152 (67\%) of the countries present a penetration higher than 50\% and 25\%, respectively.

\begin{table}[t]
\begin{tabular}{llll}
Code & Country                  & MAU penetration & DAU Penetration \\
AU   & Australia                & 71,42\%         & 55,00\%         \\
AT   & Austria                  & 50,25\%         & 36,25\%         \\
BE   & Belgium                  & 65,00\%         & 49,72\%         \\
BG   & Bulgaria                 & 54,28\%         & 41,19\%         \\
HR   & Croatia                  & 50,84\%         & 40,15\%         \\
CY   & Cyprus                   & 83,43\%         & 64,09\%         \\
CZ   & Czechia                  & 53,32\%         & 39,32\%         \\
DK   & Denmark                  & 71,03\%         & 57,30\%         \\
EE   & Estonia                  & 57,33\%         & 43,25\%         \\
FI   & Finland                  & 59,65\%         & 44,21\%         \\
FR   & France                   & 58,35\%         & 41,75\%         \\
DE   & Germany                  & 45,50\%         & 31,93\%         \\
GR   & Greece                   & 59,20\%         & 44,77\%         \\
HU   & Hungary                  & 61,95\%         & 49,01\%         \\
IE   & Ireland                  & 65,54\%         & 51,19\%         \\
IT   & Italy                    & 57,80\%         & 45,35\%         \\
LV   & Latvia                   & 52,45\%         & 39,50\%         \\
LT   & Lithuania                & 65,23\%         & 48,36\%         \\
LU   & Luxembourg               & 61,72\%         & 48,05\%         \\
MT   & Malta                    & 90,83\%         & 73,68\%         \\
NL   & Netherlands              & 63,09\%         & 47,15\%         \\
NO   & Norway                   & 70,65\%         & 57,76\%         \\
PL   & Poland                   & 50,15\%         & 36,35\%         \\
PT   & Portugal                 & 67,47\%         & 52,97\%         \\
RO   & Romania                  & 56,80\%         & 42,27\%         \\
SK   & Slovakia                 & 49,48\%         & 37,62\%         \\
SI   & Slovenia                 & 52,92\%         & 41,75\%         \\
ES   & Spain                    & 62,05\%         & 42,82\%         \\
SE   & Sweden                   & 72,74\%         & 57,03\%         \\
CH   & Switzerland              & 52,38\%         & 38,73\%         \\
UA   & Ukraine                  & 43,19\%         & 30,34\%         \\
GB   & United Kingdom           & 66,64\%         & 51,09\%         \\
US   & United States of America & 69,90\%         & 50,99\%        
\end{tabular}
\label{tab:FB_penetration}

\end{table}

Table \ref{tab:FB_penetration} is showing the penetration according to MAU and DAU for all EU countries, UK, US, Switzerland, Australia, Singapore and Norway. Most of the countries in the table are considering developing or have already developed contact-tracing apps.

If we consider the MAU metric the penetration ranges between 43\% (Ukraine) and 91\% (Malta). There are only 3 countries with a penetration below 50\% when using the MAU as reference. If we instead use the DAU the penetration goes from 30\% (Ukraine) and 74\% (Malta), with 10 countries above 50\% and 25 above 40\%.

We already mentioned in the introduction that the FB mobile app, which has been downloaded more that 5B times according to Google Store records, requests access to GPS and Network location. Although we can neither quantify for which portion of the citizens in each country FB is storing location information neither how many location points is storing,  but given the large penetration rate along with the access to location information requested by the FB mobile app suggests that FB alone may have a potentially valuable database for the purpose of contact tracing.

Facebook is just one among many LPs that could positively contribute with the location data they are already collecting. We could think of other big players such as Google or Microsoft that will probably have very large penetration rates as well. In addition, there are tons of other LPs with smaller penetrations rates that could sum up to the big players as well. 

The goal of this section is proving that ignoring LPs as a potential source of information for contact-tracing may constitute a big mistake towards achieving the goal of accessing to the contacts of 60\% of the citizens. Then we believe that it is extremely important that independent experts audit the quality of LPs data for contact tracing as soon as possible to understand whether they can contribute positively to the purpose of contact-tracing. If the independent auditing reveals the information is valid, LPs will have the moral and social obligation to contribute back to the society with the location data they collect from citizens to make large amounts of money.



==> Premises.tex <==
\section{Trust, Ethics and Legal considerations}

In this section we discuss whether it is reasonable to think of a potential misbehaviour of the main players involved in our solution, mainly public health authorities and BigTech companies. More than 300 researchers subscribed a letter that basically argued that only a fully privacy and decentralized solution could be used for contact-tracing purposes\footnote{https://drive.google.com/file/d/1OQg2dxPu-x-RZzETlpV3lFa259Nrpk1J/view}. The main reason exposed to strongly support a fully privacy-preserving solution is the so called \textit{function creep}. Function creep is defined as \textit{ "the gradual widening of the use of a technology or system beyond the purpose for which it was originally intended, especially when this leads to potential invasion of privacy"}. Therefore, the researchers signing that letter anticipates that it is likely that private companies and/or public health authorities misbehave and abuse the data processing purpose in case they get access to information such as user location or user social graph.
Next, we discusse our point of view to what extent it is reasonable to think public health authorities and/or Bigtech companies will misbehave, and whether that is something that exclusively apply to our solution or could also have implications for the currently adopted BT contact-tracing apps.

\subsection{Trust}

\subsubsection{Public Health Authorities}

At the design time of contact-tracing apps, there were some discussions regarding whether BT contact-tracing solutions should be centralized (e.g., Singapore approach\cite{TraceTogether}, initial approach from Germany that was finally discarded \cite{German_Solution}) or distributed (e.g., DP-3T approach\cite{DP-3T}).  The main difference in terms of privacy between the two solutions is that in the centralized one the public health authority may infer the network proximity graph of infected individuals reporting a positive to the central server. The team working on DP-3T solution openly criticized the centralized solution arguing that it leaves room for massive surveillance \cite{German_Solution_Critic}.

In democratic societies health authorities manage very sensitive information such as the medical record of their citizens that may include information about mental disorders, sexual transmission diseases, terminal diseases, etc. Based on the argument exposed above for not trusting health authorities, we should assume that it is likely they have misused sensitive data for different purposes that those they were collected for. However, we conjecture that societies trusting health authorities to handle the referred sensitive information would also trust them to handle COVID-19 related information such as the social contact graph of a user. 

\subsubsection{BigTech companies}

BigTech companies are probably the less trusted ones in the contexct of function creep. Therefore, initially it seems a bad idea involving them in any solution that has to do with COVID-19 contact-tracing. However, in the case of the pandemic these companies seems to have adopts a responsible position trying to support initiatives willing to contribute to the technological fight against the COVID19 \cite{Google_Mobility}\cite{Facebook_Disease}.

Probably, the most important contribution has been the support of Google and Apple to supportBT contact-tracing solutions inpired on the DP-3T protocol by integrating at the OS level an efficient BT exposure notification mechanism and offering an API to official contact-tracing apps from health authorities to benefit from it.  The letter cited at the beginning of this section applaud this initiative using the following text: \textit{"To aid the development of contact tracing without a centrally controlled database that holds private information on individuals, Google and Apple are developing infrastructure to enable the required Bluetooth operations in a privacy protective manner. Teams building the privacy protective schemes fully support this effort as it simplifies—and thus speeds up—the ability to develop such Apps. We applaud this initiative and caution against collecting private information on users."} 

In the case of our solution, health authorities will share users IDs (i.e., phone numbers) with BigTech companies like Facebook or Google. We will implement a K-anonymity approach in order to hinder Facebook and Google to infer the identity of infected users. Although our solution is not fully privacy-preserving, we believe companies like Facebook or Google do already have the capacity to infer infected users and our solution does not facilitates a lot this task. 

We are afraid privacy researchers and advocates will show strong concerns on our solution claiming that players like Google or Facebook will definitely exploit our solution for trying to infer the identity of infected users. Basically, that would mean they consider those BigTech companies cannot be trusted in the context of the COVID-19.  We would be extremely surprised if such a comment comes from someone that support the letter introduced before. In that letter, 300 very reputed researchers applaud an initiative where Google and Apple have developed a protocol that obtain the social contact graph of a user via BT. Currently, the protocol is being used in the context of the COVID19 pandemic for the purpose it was defined. However, the concept of function creep also applies in this case. Nobody can guarantee that in a near future Apple and Google manage to obtain the consent of users (e.g., accepting the terms of use associated to an OS update) and start using the contact-tracing for commercial purposes. Inferring the social contact graph would require few simple technical changes. First, both Apple and Google, could easily link the anonymous BT beacon frames to a unique user ID (e.g., Google user id account, phone IMEI, etc.). Second, each mobile device would need to deliver the transmitted and received BT beacon frames to an Apple/Google server along with the unique user ID. With that information from all Android (iOS) users, Google (Apple) could easily infer the social contact graph of any Android (Apple) user at any time window. In short, if someone strongly support that BigTech companies always rely on function creep, she should state that the support of Google and Apple to BT contact-tracing apps is nothing but a \textit{Trojan Horse} movement to get access to the social graph of the users, and supported by the conset of the users.

In summary, our approach is that if we do not trust BigTech companies to participate in technical contact-tracing solutions to fight the pandemic, we should ban them from all the solutions. However, we believe it would not be fair applauding their support when they back up a solution I support and claiming we cannot trust them when I do not like the proposed solution.

\subsection{Ethics}
In the context of COVID19 technological solutions, ethics would indicate if individuals from a given society would accept a certain solution regardless of the legal grounds supporting it. For instance, if they accept the fact that the identity of infected citizens is reported in a privacy-preserving manner to BigTech companies. Although, ethics is driven by subjectivity, and thus it is very hard to provide solid ethics grounds on complex issues as contact-tracing, it is known that citizens of well-established democracies use massively the services of bigtech companies even when they are aware these companies infer sensitive information such as the sexual orientation or religion preference of individual users [REF USENIX]. Based on this fact, we conjecture societies from democratic countries massively using bigtech services are very likely to ethically accept a solution as the one proposed in this paper. 

\subsection{Legal ground}

The legal dimension establishes whether there are provisions according to the existing legislation that makes a given technological solution legal or illegal. Contrary to ethics, here the debate is simpler.
In this paper we consider as reference the EU data protection regulation, i.e., GDPR [REF] . It is one of the most recent and protective laws (along with CCPA -California's data protection law- [REF]) in data protection and privacy and it applies to all EU countries including some of the oldest and most solid democracies in the world. The GDPR explicitly allows the use of personal data by public authorities to monitor epidemics \cite{ventrella2020privacy}. 

We acknowledge that the European Data Protection Board (EDPB) and other data protection authorities in Europe [REF] have supported the use of BT contact-tracing decentralized apps. However, such support happened 6 months ago. Now that it seems the implemented BT contact-tracing apps are not efficient enough to detect high risk contacts, we believe it would be reasonable to open the debate to alternative solutions that meet the GDPR ground in the context of a health and provide reasonable privacy guarantees to citizens, even if they are not fully privacy-preserving solutions.







==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release


==> Related_Work.tex <==
\section{Related Work}

Since the eruption of the COVID-19 in January 2020 we can find a proliferation of scientific studies aiming to contribute to control the spread of the virus, minimizing its negative effects and help public administrators taking informed decisions regarding the next steps to adopt. In the context of our papers there are two types of initiatives especially relevant. Initiatives using LPs data and works proposing contact-tracing solutions. 

\subsection{Location Providers Data}

Some Location Providers are collaborating by providing aggregated data to allow researchers, journalists, etc. analyzing mobility patterns during the crisis. 

Google have launched the so called \textit{COVID-19 Community Mobiliy Reports} \cite{Google_Mobility} that measures for a large number of countries and regions in the world how the mobility has been reduced in February and March 2020 using as baseline the median for each week day in the period Jan 3 - Feb 6 2020. They measure the aggregated mobility reduction for different Points of Interests (POIs) such as: retail \& recreation, grocery \& pharmacy, parks, transit stations, workplaces and residential. Although Google only  reports aggregated data, at the time of writing this paper Google had only delivered report but not the data.

Similarly, Facebook, in the context of its \textit{Facebook Data for Good} program is providing access to researchers to the so called Disease Prevention Maps \cite{Facebook_Disease}. This access is under request upon a data license agreement acceptance. This initiative provides researchers with mobility data between municipalities in a large number of countries in the world in daily basis. Facebook, contrary to Google, is offering actual data to researchers that may be of great value to understand the  impact of the measures adopted in different countries to minimize the OVID-19 expansion.


Another initiative, referred to as \textit{COVID-19 Mobility Data Network}, has been created following the spirit of a note published on Science Magazine \cite{Mobility_Data_Network} in which a group of scientists ask for aggregated mobility data to fight COVID-19. The network is formed by around 20 Universities and research centers that are using aggregated data from three companies: Facebook, Camber Systems, and Cuebiq, that serve as LPs in this project. This initiative has led to a dozen of reports in the following areas as defined in the Mobility Data Network: tools development; COVID in travellers; surveillance, severity and transmissibility; countermeasures, scenarios, and interventions; and, Ethics. This is an interesting initiative that uses aggregated location data in an interesting variety of topics. 

In this period, almost everyday we find new works using LPs data to uncover different aspects of the COVID-19 crisis. Following we provide a couple of illustrative examples of these works.

The NYT used data from Cuebiq that provides aggregated data of the distance people travelled at very granular geographical level in US [REF]. This depicted a map at the county level analyzing how the average distance travelled has been reduced in February and March. 

An MIT have used Cuebiq anonymous GPS location data from individuals that opted-in to share that data. In \cite{Esteban_Boston}, this team creates mobility patterns in the Boston area and through extensive simulations they evaluate the efficiency of different restriction measures after 100 cases are tested positive. In addition, they study the probability of occurrence of a second wave depending on the restrictions applied. In \cite{Esteban_NY}, using a sample of 567K users from New York City they measure the reduction of: the distance travelled, number of contacts, number of stays in 3rd places, etc. These works are of great value for public administrations to understand the efficiency of the adopted measures in order to take informed decisions in a potential second wave of the COVID-19. However, the location data used is again not valid to achieve the goal of our paper since it cannot be used to notify users that may be infected.

Finally, there are several public administrations worldwide that are collaborating with network operators to gain insights into citizens mobility during the COVID-19 crisis. For instance, in Spain the Statistics National Institute is collaborating with mobile network operators using aggregated information to unveil mobility patterns. This entity has launched a public portal where any user can explore mobility patterns over the COVID-19 crisis at the level of census areas \cite{INE_mapas}.

All these initiatives share in common with our approach that they rely in LP data. However, to the best of our knowledge, all the initiatives based on LP's information are currently working with aggregated data. Therefore, none of them are valid for contact-tracing. 

\subsection{Contact-tracing solutions}

The most adopted option worldwide is the development of new apps that could serve different purposes: (i) inform users about the pandemics, symptoms, and recommended measures to minimize the risk of infection, (ii) monitor infected users to guarantee they are not breaking the confinement, (iii) include COVID-19 diagnosis information including codes to relax or enforce restrictions on movement, (vi) contact-tracing. 

The first apps were launched in some Asian countries like China, South-Korea or Singapore. China and South-Korea have developed apps that collects individual geolocation of users that can be used for monitoring, contact tracing, and, even coercive purposes. For instance, the Korean app monitors infected users and delivers warnings when another user is within a 100m range of an infected person. In the case of China the app is not compulsory but is required to move between quarters, into public spaces and public transport.  The app reports information to a central database that combined geolocation data and coronavirus diagnosis information. An algorithm processes the information and issues color codes that are associated with more or less restrictions. The App is also available as a plug-in for the popular WeChat and Alipay mobile apps and has been widely adopted by citizens. While it seems these apps may have play a positive role in the virus spread contention, they rais bunch of data protection and privacy issues, and none of them aligns to the spirit of modern data protection regulations such as the General Data Protection Regulation (GDPR) ruling in all EU countries.

The Singapore App, referred to as \textit{TraceTogether} \cite{TraceTogether}, is, to the best of our knowledge, the first one that takes into account some privacy considerations and exclusively focuses on contact-tracing (thus eliminating from the equation other invasive features included in the case of China and South Korea). \textit{TraceTogether} assigns a random ID generated from the mobile phone of the user and sends/receive this ID to/from other devices with the app installed within a range up to 5m. Then, each mobile device stores a log of random IDs from the mobile devices it has been in contact with.  If a user is tested positive for COVID-19 the Ministry of Health (MOH) of Singapore sends a code to the mobile device that the user can use (this is a voluntary step from the user side) to upload the log file in her mobile device. Singapore's MOH has the capacity to map the random IDs to its associated mobile phone numbers, and thus can notify those users that have been in contact with a person that has been tested positive. Although the app in Singapore largely improves in privacy terms the apps from China and Korea, it is still revealing to the public administration the contact network of infected citizens. Many privacy advocates consider this is not acceptable and such practice may trigger massive surveillance even beyond the pandemics period. We will further discuss privacy Vs. efficiency aspects in Section X. 

The Singapore app was the first of its type. After \textit{TraceTogether} many other initiatives have appeared in the area of BT contact-tracing. 

WeTrace app is available in the Czech Republic \cite{WeTrace}. In this case the app broadcasts via BT a random ID of the user that any other device in its proximity (with the mobile app installed) stores. In this case, the ID is updated once a day to reduce the possibility of attacks that allow mapping the random ID broacasted by the app with the identity of the user. In case a user A is tested positive, she can voluntarily share this information so the app uploads all the IDs the user A has delivered to a central server.In turn, the central server pushes a notification to all the mobile devices with the app installed and deletes the information from user A. The app of other user, lets say B, computes locally whether user B stores locally some of the IDs of user A. If that is the case user B's app generates a warning about the risk contact and shows in a map where the contact took place. For enable this last functionality the app has to store for each random ID received the geolocation when that interaction took place. Compared to the solution used in Singapore, WeTrace provides more privacy guarantees since the contact information is not centralized by any entity. However, the delivery of gelolocation information to third persons may allow that someone reveals the identity of an infected person. 

A group of reputed researchers in the area of privacy have recently released a technical document and the code for a BT contact tracing protocol referred to as DP-3T \cite{DP-3T} that imposes a decentralized model that fully guarantees the privacy of the users. In this case, the protocol generates multiple random IDs instead of only one, which in addition cannot be mapped to the mobile phone number of the users. A mobile device send around one of the IDs for a given amount of time, and later shift to send a different one. As in the case of Singapore, the mobile app stores a log of all IDs it has received from mobile phones it has been in contact range. As in the case of WeTrace, if the user is tested positive it uploads a log file using an authentication code provided by the public administration in charge, into a central server (it only uploads the contacts of the last two weeks). The user will only upload the random IDs she has delivered. In turn, the users who have installed the app running the DP-3T protocol can download from the central server the list of all random IDs pushed by users tested positive. The mobile device runs locally an algorithm that defines the level of risk according to the proximity (can be estimated using the transmission power) and the time (can be estimated account the number of random ID from a COVID-19 positive user appears in the data downloaded) and recommend the user the actions to be taken. The protocol include further privacy-preserving features such the duration in which random IDs are locally stored. In contrast to WeTrace app, DP-3T does not store location information together with random IDs. We remark that DP-3T is not an app, but a protocol that any contact-tracing app can use. It is definitely a very robust solution in terms of privacy since it is fully decentralized and the contact tracing algorithm runs locally in the device of the user. Hence, the user is the only one knowing she has been exposed to an infected person, and she is the sole responsible of deciding whether she follows the recommendations or not. 

The Pan-European Privacy-Preserving Proximity Tracing (PEPP-PT) \cite{PEPP-PT} is an initiative involving more than 40 members (including several official governmental entities from EU states) that aims to deliver standards, technology, and services to countries and developers for developing proximity tracing apps. The proposed solution ambitions to be privacy-preserving and being able to trace infections across national borders. At the time of writing this paper, the PEPP-PT website stated: "\textit{In accordance with the recently published EU Toolbox, PEPP-PT currently considers two privacy-preserving approaches: “centralized” and “decentralized”, and continues to be open for further ideas for improvement that support PEPP-PT goals."} To the best of our knowledge, the first solution released in the context of the PEPP-PT was the "German" solution \cite{German_Solution} . Contrary, to the decentralized solutions like WeTrace and DP-3T, the German solution is centralized. First, it assigns a unique ID to each app installation (i.e., user) and is able to map the random IDs (shared via BT) to the user. Second, it traces contact similarly than previously described solution. The mobile device broadcasts short-term random IDs using BT and stores short-term random IDs received from other devices in its proximity. Third, a user is tested positive receives a code from the public administration that once introduced in the app allows the user to upload to a central server (managed by an authorized entity) both the random IDs generated and received. As in other solutions, the decision of uploading the information to the central server is voluntary. Fourth, once in the central server, the responsible public administration is able to map each random ID to the unique mobile app ID that generated the random ID. Fifth, the algorithm to detect the risk assessment algorithm runs on the central server. Note that, as in the case of DP-3T solution, the German solution does not define the algorithm that evaluates the risk arguing that it is out of the scope of the contact tracing technical solution, and should be defined by the appropriate experts. Once, the algorithm report the users exposed to a certain risk-level are notified through a push notification system that implements some privacy guarantees to avoid the possibility that specific OS features are able to infer which users have been notified. 

The German solution introduces two elements that reduces privacy guarantees compared to DP-3T. First, users are assigned a unique-ID. Second, the central server can reconstruct the network proximity graph of each user, since it knows all the unique-IDs that have been in proximity with an infected user. The DP-3T initiative has released a public document where they criticize the German proposal and argue that it leaves room for function creep (e.g., individuals surveillance) \cite{German_Solution_Critic}. 

Finally, Google and Apple has liaised in an initiative to implement contact-tracing in the mobile devices using Android and iOS, respectively [. This represents the vast majority of mobile devices worldwide. Apple and Google have announced that will work to improve the interoperability between Android and iOSes devices. This initiative has adopted the philosophy of DP-3T for performing the proximity tracing using short-term BT random IDs. Apple and Google have announced that they will have an interim solution by mid May that requires an app to work, but in the medium-term they aim to implement a solution that will be delivered along with OSes updates and will perform the contact-tracing globally without requiring an app. In turn, Google and Apple will let authorized public administrations app to access the random IDs the devices running their OSes store. Apple and Google have announced that contact-tracing will work in mobile devices upon user's consent. Apple and Google have shown their preference for decentralized solutions rather than centralized ones. Finally, based on the information delivered, this initiative will require of contact-tracing apps on top of them that covers the notification process, both from users tested positive to some central sever, and to users that have been in contact with infected users. There are still many open questions about this initiative that has not yet provided details about the concrete implementation.

Leaving apart the privacy discussion all the described solutions are similar for the task of proximity tracing. They basically exploits the benefits of BT for direct proximity contact. In addition, all the described initiatives requires that the user installs a new app. The main concern associated with new contact-tracing solutions is that according to experts [REF  Oxford] around 60\% of the citizens in a country have to install an app (could be the sum of several apps that interoperate) to efficiently fight the COVID-19 spread.  

Let us use as reference the only large-scale deployment of a contact-tracing app, i.e. Singapore. At the time of writing this paper, around 1/6 of the citizens in Singapore have installed the app. Despite the great achievement of getting that number, this is far from enough for fighting COVID-19\cite{Singapore_fail}. The huge number of installations that new mobile apps has to achieve in order to be efficient imposes a very worrying barrier for the success of any of the described initiatives. It is a huge challenge reaching that portion of installations in free democracies where users have the choice to install/use or not any of the described solutions. Even more, installing the app is not enough. Next we cite some issues that will reduce the number of installations to the actual number of efficient installations for the goal of contact-tracing and notification of risky contacts: (i) Users have also to proactively enable BT in their mobile devices to allow the proximity tracing. Some users may simply ignore how to enable it, and some others may prefer not to do it in order to save battery; (ii) In some devices, apps only work in case they are running. It is unlikely that all users has the contact-tracing mobile app they have chose open all time. If the Google-Apple initiative is widely adopted it will overcome this limitation; (iii) While getting the consent of the users multiple times across the process (e.g., consent to accept Google-Apple contact-tracing, consent to install the app, consent to share the BT random-IDs stored, etc), it is important to highlight that in each consent request it is likely that some users decides to deny the consent; (iv) In decentralized solutions, notifications are only accessible to those users receiving them. Public authorities neither manage nor keep record of such notifications. Hence, each individual is the one deciding whether she follows the recommendations to help the global public health or not. In case she ignores the recommendations nobody else will know it. In summary, new contact-tracing solutions includes multiple points where users may take an action that in practical terms reduce the number of citizens involved in the digital contact-tracing process. Therefore, for getting 60\% of the citizens actually involved in the process, it is very likely that the actual number of installations should be higher than 60\%. 

As we have already discussed, the second drawback of BT contact-tracing apps is that they are useless for indirect contact-tracing. While we do not know yet what is the actual impact of indirect contact in the case of the COVID-19, we believe it would be irresponsible completely ignoring it in the context of digital contact-tracing solutions.

This paper proposes to use readily available geolocation data from LPs to direct and indirect contact tracing. As we have shown before, only FB has a penetration beyond X\% in  more than Y countries worldwide. If we add Google, Microsoft, Twitter, and other smaller LPs it is very likely they cover almost all citizens with a mobile device. It is true that some of these players may not have high-quality location data for a portion of their registered users. Although we cannot anticipate what is the actual penetration of LPs in terms of contact-tracing, we strongly believe they could have a very important contribution towards reaching the final goal of 60\% of the citizens. Even in the case their net contribution is smaller than we expect, we believe it is worthy to explore this alternative since it is the only real option nowadays.
We propose a solution that allows performing contact-tracing with high-privacy provisions. 

Finally, we want to highlight we do not envision our proposal as an opposite solution to BT contact-tracing, but we believe both are complementary to each other. Then, while we advocate to push BT contact-tracing solutions, we believe it would be irresponsible avoid the only real existing option nowadays to explore digital contact-tracing. 












